A phase inversion benchmark for multiscale multiphase flows

A series of benchmarks based on the physical situation of "phase inversion" between two immiscible liquids is presented. These benchmarks aim at progressing toward the direct numerical simulation of two-phase flows. Several CFD codes developed in French laboratories and using either Volume-of-Fluid or Level-Set interface tracking methods are used to provide physical solutions of the benchmarks, convergence studies and code comparisons. Two typical configurations are retained, with integral scale Reynolds numbers of 13.700 and 433.000, respectively. The physics of the problem are probed through macroscopic quantities such as potential and kinetic energies, or enstrophy. In addition, scaling laws for the temporal decay of the kinetic energy are derived to check the physical relevance of the simulations. Finally the droplet size distribution is probed. Additional test problems are also reported to estimate the influence of viscous effects in the vicinity of the interface.

==> staging <==
The advection equation for $C$ is solved using a \red{Zalesak} flux-corrected scheme \cite{Zalesak79} split into successive one-dimensional steps  \cite{Bonometti} \red{in order to avoid the well-known tendency of the multidimensional version of this scheme to distort iso-C surfaces.}
Owing to the splitting procedure, the overall transport scheme is not rigorously conservative.Therefore a local mass error control which improves upon the global control technique described in  \cite{Bonometti} is employed.


The original strategy described in [70] is employed to keep this smearing within reasonable bounds.  Details may be found in [4, 70].


This modication consists in defining the interfacial region as that in which the capillary force takes non-zero values rather than that in which the volume fraction takes intermediate values. By doing so, it improves the control of the thickness of the transition region between the two fluids. 
The above strategy for the transport of $C$ makes the approach selected in JADIM intermediate between VOF and Level Set techniques: it is based on the transport
of the local volume fraction of one of the fluids but this transport is not achieved in a strictly conservative manner and no explicit reconstruction of the interface is carried out, the position of the interface being merely identified a posteriori with the isosurface $C=0.5$.




so 10-6 is a cm^3 and is indeed a suprisingly large fraction of the fluid 1 volume of 125 cm3 but since in 256^3 the cell volume is 10-3 / 2^24 = 0.0625 10-9 m3  = 6.25 10-5 cm^3
$

==> staging_ <==
The advection equation for $C$ is solved using a \red{Zalesak} flux-corrected scheme [?] split into successive one-dimensional steps [70] in order to avoid the well-known tendency of the multidimensional version of this scheme to distort iso-C surfaces.
Owing to the splitting procedure, the overall transport scheme is not rigorously conservative.Therefore a local mass error control which improves upon the global control technique described in [70] is employed. 
